The Butterfly Effect of Model Editing: Few Edits Can Trigger Large Language Models Collapse

Although model editing has shown promise in revising knowledge in Large Language Models (LLMs), its impact on the inherent capabilities of LLMs is often overlooked. In this work, we reveal a critical phenomenon: even a single edit can trigger model collapse, manifesting as significant performance degradation in various benchmark tasks. However, benchmarking LLMs after each edit, while necessary to prevent such collapses, is impractically time-consuming and resource-intensive. To mitigate this, we propose using perplexity as a surrogate metric, validated by extensive experiments demonstrating changes in an edited model's perplexity are strongly correlated with its downstream task performances. We further conduct an in-depth study on sequential editing, a practical setting for real-world scenarios, across various editing methods and LLMs, focusing on hard cases from our previous single edit studies. The results indicate that nearly all examined editing methods result in model collapse after only few edits. To facilitate further research, we have utilized GPT-3.5 to develop a new dataset, HardEdit, based on those hard cases. This dataset aims to establish the foundation for pioneering research in reliable model editing and the mechanisms underlying editing-induced model collapse. We hope this work can draw the community's attention to the potential risks inherent in model editing practices.

==> Association.tex <==
\pgfplotsset{
axis background/.style={fill=gallery},
grid=both,
  xtick pos=left,
  ytick pos=left,
  tick style={
    major grid style={style=white,line width=1pt},
    minor grid style=bgc,
    draw=none
    },
  minor tick num=1,
  ymajorgrids,
	major grid style={draw=white},
	y axis line style={opacity=0},
	tickwidth=0pt,
}


\begin{figure*}[ht]
\centering
    \begin{tikzpicture}[scale=0.5]
	\begin{groupplot}[
	    group style={group size=3 by 1,
	        horizontal sep = 42pt}, 
	    width=0.5\textwidth,
	    height=0.4\textwidth,
	    xlabel=\large Perplexity Values,
        ylabel=Acc,
        xticklabels={68.39, 124.19, 536.95, 1136.56, 4320.67, 8878.37， 50370.38},
        xtick={0, 1, 2, 3, 4, 5, 6},
        ymajorgrids,
        major grid style={draw=white},
        y axis line style={opacity=0},
        tickwidth=0pt,
        yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
        },
        scaled y ticks=false,
        every axis title/.append style={at={(0.1,0.8)},font=\bfseries}
	    ]
		\nextgroupplot[
		legend style = {
		  font=\small,
          draw=none, 
          fill=none,
          column sep = 1pt, 
          /tikz/every even column/.append style={column sep=5mm},
          legend columns = -1, 
          legend to name = grouplegend},
		title=GPT-2-XL, 
		]
         \addplot[thick,color=mine_green,mark=triangle*] coordinates {
        (0, 0.4461)
        (1, 0.2325)
        (2, 0.2158)
        (3, 0.0324)
        (4, 0.0012)
        (5, 0.0004)
        (6, 0,0002)
        }; \addlegendentry{LAMBADA}
        \addplot[thick,color=mine_blue,mark=*] coordinates {
        (0, 0.5089)
        (1, 0.4113)
        (2, 0.4154)
        (3, 0.2951)
        (4, 0.2830)
        (5, 0.2722)
        (6, 0.2668)
        };\addlegendentry{Hellaswag}
        \addplot[thick,color=mine_red,mark=diamond*] coordinates {
        (0, 0.7084)
        (1, 0.6872)
        (2, 0.6523)
        (3, 0.5588)
        (4, 0.5555)
        (5, 0.5484)
        (6, 0.5294)
        };\addlegendentry{PIQA}
        
        \nextgroupplot[
        title=GPT-J]
         \addplot[thick,color=mine_green,mark=triangle*] coordinates {
          (0, 0.6136)
        (1, 0.3233)
        (2, 0.1129)
        (3, 0.0652)
        (4, 0.0037)
        (5, 0.0000)
        (6, 0.0000)
        };
        
        \addplot[thick,color=mine_blue,mark=*] coordinates {
          (0, 0.6625)
        (1, 0.6479)
        (2, 0.4495)
        (3, 0.4012)
        (4, 0.2785)
        (5, 0.2631)
        (6, 0.2685)
        };

        \addplot[thick,color=mine_red,mark=diamond*] coordinates {
          (0, 0.7541)
        (1, 0.7421)
        (2, 0.6224)
        (3, 0.5822)
        (4, 0.5446)
        (5, 0.5326)
        (6, 0.5261)
        };
        
        \nextgroupplot[
        title=Llama2-7b]
         \addplot[thick,color=mine_green,mark=triangle*] coordinates {
        (0, 0.6814)
        (1, 0.1300)
        (2, 0.0006)
        (3, 0.0014)
        (4, 0.0008)
        (5, 0.0014)
        (6, 0.0000)
        };
        
        \addplot[thick,color=mine_blue,mark=*] coordinates {
        (0, 0.7598)
        (1, 0.6818)
        (2, 0.5090)
        (3, 0.2812)
        (4, 0.2626)
        (5, 0.2638)
        (6, 0.2599)
        };

        \addplot[thick,color=mine_red,mark=diamond*] coordinates {
        (0, 0.7845)
        (1, 0.7307)
        (2, 0.6415)
        (3, 0.5457)
        (4, 0.5196)
        (5, 0.5326)
        (6, 0.5294)
        };
        
	\end{groupplot}
\node at ($(group c1r1) + (370pt, 95pt)$) {\ref{grouplegend}};
\end{tikzpicture}

    \caption{Extensive Collapse Phenomenon}
    \label{Fig_Extensive_Collapse}
\end{figure*}



  


==> Extent_Collapse_Fig.tex <==
\pgfplotsset{
axis background/.style={fill=gallery},
grid=both,
  xtick pos=left,
  ytick pos=left,
  tick style={
    major grid style={style=white,line width=1pt},
    minor grid style=bgc,
    draw=none
    },
  minor tick num=1,
  ymajorgrids,
	major grid style={draw=white},
	y axis line style={opacity=0},
	tickwidth=0pt,
}


\begin{figure*}[ht]
\centering
    \begin{tikzpicture}[scale=0.5]
	\begin{groupplot}[
	    group style={group size=4 by 3,
	        horizontal sep = 42pt}, 
	    width=0.5\textwidth,
	    height=0.4\textwidth,
	    xlabel=\large Edit Times,
        ylabel=Perplexity Values,
        xticklabels={0, 10, 20, 30, 40, 50},
        xtick={0, 1, 2, 3, 4, 5},
        ymajorgrids,
        major grid style={draw=white},
        y axis line style={opacity=0},
        tickwidth=0pt,
        yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
        },
        scaled y ticks=false,
        every axis title/.append style={at={(0.1,0.8)},font=\bfseries}
	    ]
		\nextgroupplot[
		legend style = {
		  font=\small,
          draw=none, 
          fill=none,
          column sep = 1pt, 
          /tikz/every even column/.append style={column sep=5mm},
          legend columns = -1, 
          legend to name = grouplegend},
		title=FT+GPT-2, 
		]
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
        (0, 1.8349926037330297)
        (1, 2.0800475775595473)
        (2, 4.153097609928517)
        (3, 3.775525531416595)
        (4, 4.690815155022235)
        (5, 4.925382499744859)
        }; \addlegendentry{Normal Cases}
        \addplot[thick,color=flamingo,mark=*] coordinates {
        (0, 1.8349926037330297)
        (1, 2.3431357526888776)
        (2, 4.35035442282019)
        (3, 4.492148988756076)
        (4, 4.615731210828967)
        (5, 4.608974338943906)
        };\addlegendentry{Hard Cases}
        
        \nextgroupplot[
        title=MEND+GPT-2]
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (0, 1.8349926037330297)
        (1, 5.079458210211661)
        (2, 5.213325518731122)
        (3, 5.394671598467645)
        (4, 5.443642154943337)
        (5, 5.508394834186697)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (0, 1.8349926037330297)
        (1, 5.021120885419502)
        (2, 5.598985639113134)
        (3, 5.786581671109532)
        (4, 5.704836352827301)
        (5, 5.665029223469695)
        };
        
        \nextgroupplot[title=ROME+GPT-2]
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
        (0, 1.8349926037330297)
        (1, 1.8351644280309387)
        (2, 1.8365062505873473)
        (3, 1.8390682612009788)
        (4, 1.8422244945481894)
        (5, 1.8481837714561062)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
        (0, 1.8349926037330297)
        (1, 5.257119012434592)
        (2, 5.439196846673717)
        (3, 5.169480505687279)
        (4, 5.124878522518401)
        (5, 7.552455404540906)
        };
        
        \nextgroupplot[title=MEMIT+GPT-2]	
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
        (0, 1.8349926037330297)
        (1, 1.8350094834151849)
        (2, 1.8352564099417263)
        (3, 1.835508125122048)
        (4, 1.8356719551974239)
        (5, 1.8359297211143901)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
        (0, 1.8349926037330297)
        (1, 1.8369328753017184)
        (2, 1.8380890152835867)
        (3, 1.8398766981906838)
        (4, 1.8413152843877607)
        (5, 1.8441950193575163)
        };
        
        
        \nextgroupplot[
        title=FT+GPT-J,
        ylabel=Perplexity Values]
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (0, 1.7019132112123438)
        (1, 1.8034547218702712)
        (2, 1.8784160615589525)
        (3, 2.1032018326484647)
        (4, 2.234179176109935)
        (5, 2.3198264261413155)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (0, 1.7019132112123438)
        (1, 1.82006156590004)
        (2, 2.4954253885140862)
        (3, 2.104006607465171)
        (4, 2.128231263891013)
        (5, 1.9991279348748314)
        };
        
        \nextgroupplot[
        title=MEND+GPT-J,
        ylabel=Perplexity Values]
		\addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (0, 1.7019132112123438)
        (1, 3.1589931044918274)
        (2, 4.48918425910019)
        (3, 4.124749905940776)
        (4, 3.632968356534176)
        (5, 3.9460772288920465)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (0, 1.7019132112123438)
        (1, 3.1201949272544725)
        (2, 3.7096413330976854)
        (3, 3.4989305687046524)
        (4, 3.8364949144117464)
        (5, 4.312112375665962)
        };
        
        \nextgroupplot[
        title=ROME+GPT-J,
        ylabel=Perplexity Values]
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (0, 1.7019132112123438)
        (1, 1.7019512168120754)
        (2, 1.7018321778601042)
        (3, 1.7026338672770045)
        (4, 1.7023608540065434)
        (5, 1.702794017964693)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (0, 1.7019132112123438)
        (1, 6.739430965093368)
        (2, 5.955079533423719)
        (3, 6.770837945931003)
        (4, 6.702793178501625)
        (5, 7.094452695518626)
        };
        
        \nextgroupplot[
        title=MEMIT+GPT-J,
        ylabel=Perplexity Values]
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (0, 1.7019132112123438)
        (1, 1.7019735730718248)
        (2, 1.7022060949814302)
        (3, 1.702489463574041)
        (4, 1.7024651780960725)
        (5, 1.7028100476777956)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (0, 1.7019132112123438)
        (1, 1.730749514126909)
        (2, 1.8537491456482371)
        (3, 2.8526021669265633)
        (4, 9.507658646191368)
        (5, 8.969896915798229)
        };

        \nextgroupplot[
        title=FT+Llama,
        ylabel=Perplexity Values]
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (0, 1.5711262770843115)
        (1, 1.6519326748828416)
        (2, 2.0455465870578178)
        (3, 2.4197627974367615)
        (4, 2.564972366137125)
        (5, 2.7431546213093982)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (0, 1.5711262770843115)
        (1, 1.7017843135877222)
        (2, 1.8452797187957646)
        (3, 2.3001439118737053)
        (4, 2.4666818590270787)
        (5, 2.6668675468238145)
        };

        \nextgroupplot[
        title=MEND+Llama,
        ylabel=Perplexity Values]
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (0, 1.5711262770843115)
        (1, 2.2084373851463655)
        (2, 5.276867629920992)
        (3, 6.580115815026821)
        (4, 8.775376351533192)
        (5, 8.55077867465155)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (0, 1.5711262770843115)
        (1, 2.064257440185523)
        (2, 4.654449466803819)
        (3, 5.761502216246751)
        (4, 7.879826163626375)
        (5, 10.364902268040746)
        };

        \nextgroupplot[
        title=ROME+Llama,
        ylabel=Perplexity Values]
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (0, 1.5711262770843115)
        (1, 1.5709039846059667)
        (2, 1.5708150341753928)
        (3, 1.571050764120299)
        (4, 1.5707822627797032)
        (5, 1.5714446648217286)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (0, 1.5711262770843115)
        (1, 3.551312722684355)
        (2, 4.737603354267447)
        (3, 5.067101703171905)
        (4, 5.285450807127539)
        (5, 5.594871546008)
        };

        \nextgroupplot[
        title=MEMIT+Llama,
        ylabel=Perplexity Values]
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (0, 1.5711262770843115)
        (1, 1.5720864830866828)
        (2, 1.5725803711550095)
        (3, 1.5744459741996055)
        (4, 1.5818286209882821)
        (5, 1.5844105503753727)
        };
        
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (0, 1.5711262770843115)
        (1, 2.4678773490737016)
        (2, 7.412725668577965)
        (3, 6.59152881303586)
        (4, 7.002982038418408)
        (5, 7.167508403621489)
        };
        
	\end{groupplot}
\node at ($(group c1r1) + (370pt, 95pt)$) {\ref{grouplegend}};
\end{tikzpicture}

    \caption{Extensive Collapse Phenomenon}
    \label{fig_seq}
\end{figure*}  


==> Related_Works.tex <==
\subsection{Related Works}
\label{subsec:related_work}



\subsubsection{Knowledge Editing}
\label{apd_ke}
In the realm of knowledge editing, which encompasses model editing, there exists a category of parameter-preserving techniques that diverge from the direct modification of internal parameters.
These techniques predominantly focus on enhancing LLMs with external memory \cite{mitchell2022memorybased, zheng2023edit, zhong2023mquake} or additional parameters \cite{dong2022calibrating, hartvigsen2023aging, huang2023transformerpatcher}, facilitating the incorporation of new knowledge without altering the core model structure. 
SERAC \cite{mitchell2022memorybased} employs external memory to store edit information and trains a scope classifier to retrieve the relevant edit based on the input, thereby serving as context to alter the behavior of LLMs. 
T-Patcher \cite{huang2023transformerpatcher} introduces additional key-value pairs into MLP modules of LLMs to incorporate specific knowledge without modifying unrelated information. 

The side effects resulting from these approaches are extrinsic to the models and, as such, fall outside the purview of our research discussion.

\subsubsection{Evaluation of Edited Models} 
Establishing fast and reliable methods for assessing whether edited models maintain their original capabilities and extraneous knowledge is a a pivotal concern in the field of model editing. 
Locality, also known as Specificity, is a prevalent metric used to evaluate whether post-edit models continue to provide accurate responses to queries that fall outside the scope of the edits \cite{meng2023locating, yao2023editing, meng2023massediting, yu2023melo}.
\citet{hoelscherobermaier2023detecting} claim a limitation in the currently used Specificity metric, which focuses only on model responses to given prompts, and propose using KL divergence to measure changes in the full probability distribution of model outputs. 
\citet{yao2023editing} evaluate GPT-J models that are sequentially edited 100 times using various editing algorithms on a commonsense task; however, the method is not widely adopted for the complexity of assessment and the limitation of a single task.
Recently, \citet{gu2024model} and \citet{gupta2024model} have assessed the impact of editing on downstream tasks performance of models, demonstrating that massive edits can disrupt models' general capabilities.

However, current evaluation methodologies either fail to provide a comprehensive assessment, focusing solely on localized behavioral changes within the model, or are constrained by the complexity and high costs of evaluation, rendering them impractical for massive edits. 
Our research aims to capture the comprehensive changes in the model’s capabilities during extensive editing in practical applications.

\subsubsection{Side Effects of Model Editing}
\label{apd_SideEffect}
Existing explorations of side effects primarily concentrate on the non-robust behaviors of model associated with editing. 
\citet{gu2024model} and \citet{gupta2024model} reveal that extensive edits can induce obvious side effects on models' general abilities.

Distinct from these works, our research investigates the impacts of editing on the overall capabilities of the model and identify prevalent model collapse caused by few edits.

we focus on exploring the possibility of model collapse caused by a small number of edits and how to efficiently detect potential collapses in practical applications.


Distinct from contemporaneous works \cite{gu2024model, gupta2024model} focusing on the impact of large-scale edits on models, we focus on exploring the possibility of model collapse caused by a small number of edits and how to efficiently detect potential collapses in practical applications.

